Continual Learning for Image Segmentation with Dynamic Query

Image segmentation based on continual learning exhibits a critical drop of performance, mainly due to catastrophic forgetting and background shift, as they are required to incorporate new classes continually. In this paper, we propose a simple, yet effective Continual Image Segmentation method with incremental Dynamic Query (CISDQ), which decouples the representation learning of both old and new knowledge with lightweight query embedding. CISDQ mainly includes three contributions: 1) We define dynamic queries with adaptive background class to exploit past knowledge and learn future classes naturally. 2) CISDQ proposes a class/instance-aware Query Guided Knowledge Distillation strategy to overcome catastrophic forgetting by capturing the inter-class diversity and intra-class identity. 3) Apart from semantic segmentation, CISDQ introduce the continual learning for instance segmentation in which instance-wise labeling and supervision are considered. Extensive experiments on three datasets for two tasks (i.e., continual semantic and instance segmentation are conducted to demonstrate that CISDQ achieves the state-of-the-art performance, specifically, obtaining 4.4% and 2.9% mIoU improvements for the ADE 100-10 (6 steps) setting and ADE 100-5 (11 steps) setting.

==> COCO_40_4.tex <==
% attention

\centering
\setlength{\tabcolsep}{1.3mm}
\footnotesize
% 	\def\x{{$\footnotesize \times$}}
\begin{tabular}{ l|c||ccccccccccc|c} 
\toprule
\multirow{2}*{\textbf{Method}}&
\multirow{2}*{\textbf{Queries}}& \multicolumn{12}{c}{\textbf{COCO 40-8 (6 steps)}}  \\
 & &  \textit{0-40} & \textit{41-44} & \textit{45-48}  & \textit{49-52} & \textit{53-56} & \textit{57-60} & \textit{61-64} & \textit{65-68} & \textit{69-72} & \textit{73-76} & \textit{77-80} & \textit{mAP}   \\ 
\midrule
Joint Training~(offline) & 100 & - & - & 43.7  & - & -& - & -& - & - & 43.7 & - & -\\
Joint Training~(offline) & 200 & - & - & 43.7  & - & -& - & -& - & - & 43.7 & - & -  \\
% Joint Training~$^{\star}$ &   100 & - & - & - & - & - & - & - & - & - & - & - & - \\
% MiB~$^{\star}$ & 100 & - & - & - & - & - & - & - & - & - & - & - & - \\ 
% PLOP~$^{\star}$ & 100 & - & - & - & - & - & - & - & - & - & - & - & - \\ 
% SSUL~$^{\star}$ & 100 &- & - & - & - & - & - & - & - & - & - & - & - \\
% \midrule
\textbf{CiSDQ} (step \#0) & 100 & 29.5 & - & 14.7 & 29.5 & - & - & 14.7 & 29.5 & - & - & - & -  \\
\textbf{CiSDQ} (step \#1) & 100\dt{$+100/n$} & 22.9 & 24.5 & 23.7 & -& - & -& - & - & - & - & - & -  \\
\textbf{CiSDQ} (all steps) & 200 & 22.9 & 24.5 & 23.7 & - & -& - & - & - & - & - & - \\
% \midrule
% Joint Training~$^{\star}$ &  200 & - & - & - & - & - & - & - & - & - & - & - & - \\
% \midrule
% \textbf{CiSDQ} (ours) & 200\dt{$+200/n$} &  - & - & - & - & - & - & - & - & - & - & - & -\\

\bottomrule
\end{tabular}


==> COCO_instance.tex <==
% attention

\centering
\setlength{\tabcolsep}{1.3mm}
\footnotesize
% 	\def\x{{$\footnotesize \times$}}
\begin{tabular}{ l||cc|c||cc|c||cc|c||cc|c } 
\toprule
\multirow{2}*{\textbf{Method}}&
% \multirow{2}*{\textbf{Queries}}&
\multicolumn{3}{c||}{\textbf{COCO 40-40 (2 steps)}} & \multicolumn{3}{c||}{\textbf{COCO 40-8 (6 steps)}} & \multicolumn{3}{c||}{\textbf{COCO 40-4 (11 steps)}} & \multicolumn{3}{c}{\textbf{COCO 60-20 (2 steps)}}\\
 &  &  \textit{0-40} & \textit{41-80} & \textit{all} & \textit{0-40} & \textit{41-80} & \textit{all} & \textit{0-40} & \textit{41-80} & \textit{all} & \textit{0-40} & \textit{41-80} & \textit{all} \\ 
\midrule
Joint Training &  - & - & 43.7 & - & - & 43.7 & - & - & 43.7 & - & - & 43.7\\
% Joint Training~$^{\star}$ &   100 & - & - & - & - & - & - & - & - & - & - & - & - \\
% MiB~$^{\star}$ & 100 & - & - & - & - & - & - & - & - & - & - & - & - \\ 
% PLOP~$^{\star}$ & 100 & - & - & - & - & - & - & - & - & - & - & - & - \\ 
% SSUL~$^{\star}$ & 100 &- & - & - & - & - & - & - & - & - & - & - & - \\
% \midrule
\textbf{CiSDQ} (ours) & - & - & - & - & - & - & - & - & - & - & - & -\\
% \midrule
% Joint Training~$^{\star}$ &  200 & - & - & - & - & - & - & - & - & - & - & - & - \\
% \midrule
% \textbf{CiSDQ} (ours) & 200\dt{$+200/n$} &  - & - & - & - & - & - & - & - & - & - & - & -\\

\bottomrule
\end{tabular}


==> loss_weight.tex <==


\centering
\setlength{\tabcolsep}{0.4mm}
\tiny
\begin{tabular}{cccc|ccc}
$\lambda_1 (\mathcal{L}_q)$ & $\lambda_2 (\mathcal{L}_c)$ & $\lambda_3 (\mathcal{L}_m)$ & $\lambda_4 (\mathcal{L}_{pod})$ &  1-100 & 101-150 & \textit{all} \\
\hline
0.2 & 5 & 150 & 100 & 44.9 & 13.0 & 34.3 \\
0.2 & 5 & 300 & 100 & 45.3 & 12.9 & 34.5 \\
0 & 5 & 300 & 100 & 38.7 & 15.6 & 31.0 \\
10 & 5 & 300 & 100 & 46.8 & 15.1 & 36.2 \\
1 & 5 & 300 & 0 & 41.3 & 17.9 & 33.5\\
1 & 5 & 300 & 10 & 43.5 & 17.7 & 34.9\\
1 & 5 & 300 & 1000 & 47.1 & 12.1 & 35.4\\
1 & 5 & 300 & 100 & 46.2 & 17.6 & 36.7\\
\end{tabular}


==> pkd.tex <==


\centering
\setlength{\tabcolsep}{0.4mm}
\tiny
\begin{tabular}{c|ccc}
KD &  1-100 & 101-150 & \textit{all} \\
\hline
Pseudo label &  &  & \\
Prediction-KD &  &  & \\
\end{tabular}
